CEV-LM: Controlled Edit Vector Language Model for Shaping Natural Language Generations

As large-scale language models become the standard for text generation, there is a greater need to tailor the generations to be more or less concise, targeted, and informative, depending on the audience/application. Existing control approaches primarily adjust the semantic (e.g., emotion, topics), structural (e.g., syntax tree, parts-of-speech), and lexical (e.g., keyword/phrase inclusion) properties of text, but are insufficient to accomplish complex objectives such as pacing which control the complexity and readability of the text. In this paper, we introduce CEV-LM - a lightweight, semi-autoregressive language model that utilizes constrained edit vectors to control three complementary metrics (speed, volume, and circuitousness) that quantify the shape of text (e.g., pacing of content). We study an extensive set of state-of-the-art CTG models and find that CEV-LM provides significantly more targeted and precise control of these three metrics while preserving semantic content, using less training data, and containing fewer parameters.

==> sections/old/methodology.tex <==
\section{Prototype-then-edit Model}
\label{sec:ne_model}

\citet{guu2018generating} introduce a novel unconditional generative model that samples a ``prototype'' sentence from the training corpus and edits it using a randomly sampled edit vector. The authors find that within the Yelp restaurant review corpus, 70\% of the test set is within a Jaccard distance of 0.5 of a training set sentence, implying that a neural editor with smooth and consistent edits should capture the test set. There are two significant constraints for the edit model:
\begin{itemize}
    \item \textbf{Semantic Smoothness}: Edits should change the semantics of text by a small amount and, when stacked together, create a larger change.
    \item \textbf{Consistent Edit Behavior}: The edit vector, $z$, should control the change in a sentence such that when applied to different sentences, the edits are semantically analogous.
\end{itemize}

% We provide details into how \cite{guu2018generating} define their model. 
The likelihood of a sentence is formulated as $p(x) = \sum_{x' \in \mathcal{X}} p(x | x') p(x')$ where $x'$ is prototype sentence and $x$ is the generated sentence. We define $p(x | x') = \mathbb{E}_{z \sim p(z)} [p_{edit}(x | x', z)]$ where $p_{edit}(x | x', z)$ is our neural editor. A sum over all prototypes $x'$ is expensive so we only sum over the $x'$ that are lexically similar to $x$ - a lexical similarity neighborhood, $\mathcal{N}(x)$. 


% $$p(x) = \sum_{x' \in \mathcal{X}} p(x | x') p(x')$$

% where $x'$ is prototype sentence, $x$ is the generated sentence, and  $p(x | x') = \mathbb{E}_{z \sim p(z)} [p_{edit}(x | x', z)]$. However, since this requires a sum over all prototypes $x'$, the authors only sum over the $x'$ that are lexically similar to $x$. They create a lexical similarity neighborhood:

% $$\mathcal{N}(x) = \{x' \in \mathcal{X} : d_J(x, x') < 0.5\}$$

% where $d_J$ is the Jaccard distance. The  model is trained by maximizing the marginal likelihood, $p(x)$, with gradient ascent. However, $p(x|x')$ has no closed-form solution, which is solved by lower bounding the expectation with the evidence lower bound (ELBO) \cite{kingma2013auto} 

% Ultimately, 
The model features three main components: a neural editor $p_{edit}(x | x', z)$, an inverse neural editor $q(z | x', x)$, and an edit prior $p(z)$. Note that the neural editor and inverse neural editor combine to form a VAE. The neural editor is implemented as a sequence-to-sequence model with attention, where given $x'$ as input and $z$, which is concatenated to the input of the decoder at each step, it ultimately generates $x$. The edit prior $z = z_{norm} \cdot z_{dir}$ where $z_{norm}$, the strength of the edit, is drawn from $\mathcal{U}(0,10)$ and $z_{dir}$, the direction of the edit, is sampled from a uniform distribution on the unit sphere. The inverse neural editor is given the edit pair $(x, x')$ and must infer the edit vector $z$. The difference between $x$ and $x'$ is represented as

$$f(x, x') = \sum_{w \in I} \Phi(w) \oplus \sum_{w \in D} \Phi(w)$$

where $I = x \setminus x'$ (\ie the set of words added to $x'$), $D = x \setminus x'$ (\ie the set of words deleted from $x'$), and $\Phi(w)$ is the GloVe \cite{pennington2014glove} vector for $w$. The inverse neural editor outputs a perturbed version of $f(x, x')$ as the edit vector, as follows:

$$q(z_{dir} | x', x) = \text{vMF}(f_{dir}, \kappa)$$
$$q(z_{norm} | x', x) = \mathcal{U}(f_{norm}, f_{norm} + \epsilon)$$

where $f_{norm} = \min(\|f\|, 10 - \epsilon)$ and $f_{dir} = \frac{f}{f_{norm}}$. Let $\text{vMF}(\mu, \kappa)$ be a von-Mises Fisher distribution where $\mu$ is the mean vector, and $\kappa$ is the concentration parameter.\footnote{$\kappa$ controls the rate of decay as the log-likelihood of a point decays linearly with the cosine similarity to $\mu$ in vMF distributions}

\section{Controllable Edit Vectors}
\label{sec:ne_edits}

% In order to introduce a control mechanism for our target features, we alter two aspects of the prototype-then-edit model: neighborhood creation and edit vector perturbation.
To exhibit control over our target attributes, we alter the prototype-then-edit model in two ways: neighborhood creation and edit vector perturbation. The former constrains the edit prior to edit vectors that demonstrate the desired change in attribute, within some tolerance $\epsilon$. The latter encourages a perturbation to the edit vector in the desired direction to compensate for $\epsilon$.

\textbf{Constrained Neighborhood Creation}: The model's behavior is heavily constrained by the lexical similarity condition in the creation of the neighborhood. By creating an additional constraint on the target attribute, we can ensure that edit vectors drawn from $p(z)$ correspond to a specified change in that attribute. More formally, we define the neighborhood as

\begin{align*}
    \mathcal{N}_{\Delta}(x) &= \{x' \in \mathcal{X} : d_J(x, x') < 0.5, \\
                            &  \hspace{0.3in} |(s(x) - s(x')) - \Delta| \leq \epsilon \}
\end{align*}

where $s(\cdot)$ computes the target attribute given text, $\delta$ is a desired change in the target attribute, and $\epsilon$ is the tolerance.
% Note that direction is enforced with $(s(x) - s(x'))$.

\textbf{Controlled Edit Vector Peturbation}: We hypothesize that by altering the magnitude of $z_{norm}$ and the direction $z_{dir}$, we can control the strength and behavior of the edit vector. Expressly, we can condition the formulation of the inverse neural editor on the target attribute by defining $q(z_{norm} | x', x) = \mathcal{N}(\Delta, 1) \cdot \mathcal{U}(f_{norm}, f_{norm} + \epsilon)$, where $\mathcal{N}$ is the normal distribution, $\mathcal{U}$ is the uniform distribution, and $\Delta$ is the desired change in the target attribute.


==> sections/results_fig.tex <==
\section{Results}
\label{sec:ne_results}

% \footnote{The variance across runs is generally negligible for each metric (\eg $0.005$ for BERTScore) and thus we omit it from tables, only reporting the averaged metric.} 

\begin{figure*}[]
  \centering
  \caption{Percent errors for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. We find that our approaches (\textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) show significantly more control over all control conditions across nearly all target deltas.}
  \includegraphics[width=\textwidth]{figs/delta_comps.pdf}
  \label{fig:errors}
  \vspace{-15px}
\end{figure*}

In this section, we evaluate \textsc{Cev-LM} on the strength of control (\Cref{subsec:control_eval}) as well as the relevance to the original text (\Cref{subsec:semantic_sim} and~\Cref{subsec:lexical_sim}). In \Cref{subsec:tolerance}, we discuss tuning the tolerance hyperparameter and in~\Cref{subsec:tolerance}, the effect of the data distribution on training. We provide qualitative results in~\Cref{subsec:qualitative}.

\subsection{Control Evaluation}
\label{subsec:control_eval}

We use the out-of-the-box edit-then-prototype (\textsc{Edit-then-Prototype}) model to provide a baseline $\Delta$ for all evaluations (except in~\Cref{fig:errors}, as the error would almost always be $100\%$). We run all baselines three times and report the average.

~\Cref{fig:errors} show the percent error of each approach across various target deltas, while~\Cref{fig:bleu_bert} shows the BERT and BLEU scores. We find that \textsc{Cev-LM} exhibits significantly greater control of $\Delta$ over the baseline approaches while preserving lexical and semantic similarity across all three attributes and all target deltas.

The baselines generally yield fluent but not controlled text. GPT-3 often generates texts with minimal change in attribute (\ie $\Delta = 0$), showing it cannot understand these nonstandard control conditions through few-shot learning. Conversely, prefix-tuning can replicate the attributes somewhat well but falls short due to neural hallucinations and poor-quality text. In low-resource scenarios (\ie high target deltas and fewer training samples), prefix-tuning led to significant over- or under-fitting; thus, we omit the results. In many cases, MuCoCO and SSD-LM perform poorly in terms of percent error but sometimes outperform or perform on par with our approaches. While we cannot fully explain this behavior, we hypothesize that the data distribution of $\Delta$ in $\mathcal{N}(x)$ plays a significant role. In some cases, we see strong results with both \textsc{Cev-LM} modifications, indicating that combining the modifications is beneficial with certain attributes and when $\epsilon$ is tuned. Specifically, volume consistently benefits from controlled edit vector perturbation, while speed and circuitousness show conflicting results. We find that circuitousness has much larger errors on average, likely due to the dependency on computing the shortest path.

% We plot these distributions in~\Cref{fig:feature_distr} and provide further reasoning in~\Cref{appendix:data_dist}.
\subsection{Semantic Similarity}
\label{subsec:semantic_sim}

In the first subfigure of~\Cref{fig:bleu_bert}, we report the BERT Scores of all approaches across various target deltas for each nonstandard control condition. We observe that \textsc{Cev-LM} consistently outperforms the other approaches while performing about on par with the edit-then-prototype baseline. This demonstrates that our approach preserves semantic similarity while significantly changing the speed, volume, or circuitousness of the text (also seen in~\Cref{tab:eval}). As the target delta increases, the BERT Score of our approach tends to decrease. We explain this phenomenon further in~\Cref{subsec:data_dist}.

% ================================================================================================
\begin{figure*}[]
  \centering
  \caption{BLEU and BERT (F1) scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
  \includegraphics[width=\textwidth]{figs/bert_comps.pdf}
  \includegraphics[width=\textwidth]{figs/bleu_comps.pdf}
  \label{fig:bleu_bert}
  \vspace{-15px}
\end{figure*}
% ================================================================================================

% \begin{figure*}[]
%   \centering
%   \caption{BERT Scores (F1) for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
%   \includegraphics[width=\textwidth]{figs/bert_comps.pdf}
%   \label{fig:bert}
%   \vspace{-15px}
% \end{figure*}

\subsection{Lexical Similarity}
\label{subsec:lexical_sim}

In the latter part of~\Cref{fig:bleu_bert}, we report the BLEU Scores of all approaches across various target deltas for each nonstandard control condition. We generally observe similar trends for our approaches in that BLEU score decreases as target delta increases, although to a greater scale. Since BLEU score measures lexical similarity, it is more sensitive to changes in wording, leading to a larger spread of scores. We also find that unlike before, \textsc{Cev-LM} does not clearly outperform the other approaches, which may imply that it presents semantically similar content while changing the wording. 

% \begin{figure*}[]
%   \centering
%   \caption{BLEU scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
%   \includegraphics[width=\textwidth]{figs/bleu_comps.pdf}
%   \label{fig:bleu}
%   \vspace{-15px}
% \end{figure*}

% While speed and volume perform nearly identically in~\Cref{tab:eval}, both with low errors, volume reacts much better to edit vector perturbation.

\subsection{Tolerance Tuning}
\label{subsec:tolerance}

We measure the impact of $\epsilon$ on training, testing $\epsilon = \{0.05, 0.1, 0.2\}$. When tolerance is too low, the approach overfits from the lack of training data, leading to smaller percent errors and poor similarity metrics. Including controlled perturbations to edit vectors improves similarity metrics at the cost of $\Delta$, indicating that the approach may help combat overfitting.  The effect of controlled edit vector perturbation is inconsistent across tolerance values and attributes, so we use $\epsilon = 0.1$ to provide an effective balance of control over a certain $\Delta$ and enough data for robust training. More details can be found in~\Cref{appendix:tolerance}.

% It is likely that the perturbation benefits from having $\Delta$-constrained pairs but we leave it to future work to investigate this behavior.

\subsection{Training Delta Distribution}
\label{subsec:data_dist}

We analyze the distribution of $\Delta$ in $\mathcal{N}(x)$ in~\Cref{fig:feature_distr}. The distribution is centered at 0 and denser at smaller magnitudes of $\Delta$, implying a lack of training data for larger shifts in the target attribute. This explains the general trend of increasing MAE and decreasing BLEU/BERT score as the target delta increases, seen in~\Cref{tab:eval}.

\begin{figure*}[]
  \centering
  \caption{Histogram of delta values (\ie $s(x) - s(x')$) within the Yelp Restaurant Review Corpus. The x-axis represents the difference in speed within the pairs of our created neighborhood, $\mathcal{N}(x)$, without any constraint on speed. The y-axis counts the number of pairs exhibiting the given delta in log-scale.}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/speed.pdf}}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/volume.pdf}}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/circuitousness.pdf}}
  \label{fig:feature_distr}
\end{figure*}

In~\Cref{fig:samples_vs_error}, we record the performance against the number of training samples, finding that despite fewer samples, control through low-resource training is just as successful as through high-resource training. While circuitousness is the worst-performing attribute, likely due to the complexity of capturing the shortest path-based computation, it surprisingly does worst in a high-resource setting. It is possible that the change in attribute was too small to capture, even with a high number of samples. We see some success with decreasing the number of samples by a few orders of magnitude while preserving performance, across all attributes but leave extensive investigation to future work.

\begin{figure}[]
  \centering
  \caption{The number of samples used for training versus percent error. The attribute is denoted by the shape, target delta by the color, and the border indicates that perturbation was used. Despite access to significantly fewer samples, low-resource models exhibit similar amounts of control to high-resource models.}
  \scalebox{0.7}{
  \includegraphics[width=0.68\textwidth]{figs/samples_vs_error.pdf}
  }
  \label{fig:samples_vs_error}
\end{figure}

\subsection{Qualitative Results}
\label{subsec:qualitative}

\Cref{tab:ne_speed_example,tab:ne_volume_example,tab:ne_circuitousness_example} show the generations of the \textsc{Edit-then-Prototype} Baseline, GPT-3, SSD-LM, and each of our methods (\ie \textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) with $\epsilon=0.1$ when given a target delta of $0.5$ for speed, volume, and circuitousness, respectively. 
In~\Cref{tab:ne_speed_example}, we observe that our approaches generations tend to convey the same information in a shorter span, indicating an increase in speed. GPT-3 is generally not consistent, and SSD-LM tends to stray off-topic. In~\Cref{tab:ne_volume_example}, we can see that our approach tends to add information/verbosity, indicating an increase in volume. Here, GPT-3 shows little to no change in generation, and again, SSD-LM tends to stray off-topic, hallucinating information. Lastly, in~\Cref{tab:ne_circuitousness_example}, our approach leads to more indirect descriptions. While the text is more verbose, like volume, it repeats information/words, a key facet of circuitousness. GPT-3 hardly changes the input, and SSD-LM hallucinates some information. 

In addition to qualitative observations comparing variations of our approach, ~\Cref{tab:eval} in~\Cref{appendix:perturb} shows the results of training without and with controlled edit vector perturbation, respectively, in comparison to a baseline edit-then-prototype model to show that our approach significantly changes the behavior of the edit-then-prototype model. 

% For both sequences, the generations of our modified models are much shorter while preserving content, indicating higher speed. The baseline for both prompts made minimal edits to the input sentences (\eg ``excellent'' to ``amazing''), resulting in close to no change in speed but an extremely high similarity. GPT-3 and SSD-LM both struggled to change the speed of the text and significantly strayed from the original text, sometimes changing the meaning. 

 

  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{speed}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_speed_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Speed}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: He went above and beyond in providing us excellent customer service and was extremely courteous friendly and kind.  \\
  \textbf{\textsc{Edit-then-Prototype}}: He went above and beyond in providing us with amazing customer service and was extremely courteous friendly and kind.  \\
  \textbf{GPT-3}: He was a great customer service provider. He was friendly and kind, \\
  \textbf{SSD-LM}: I was pleased that this was in line with our expectations. Suggesting the right\\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Always amazing customer service and very knowlegable staff. \\
  \textbf{\textsc{Cev-LM}}: He was knowledgable, courteous, and went provided excellent customer service.\\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: The staff is very professional and friendly \& environment is clean.  \\
  \textbf{\textsc{Edit-then-Prototype}}: The staff is very professional and likable \& the environment is clean. \\
  \textbf{GPT-3}: The staff was very professional, but not too friendly. The environment was clean, \\
  \textbf{SSD-LM}: This is a great experience! Reviews the best experience in the world. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The friendly staff is very professional \& environment is clean. \\
  \textbf{\textsc{Cev-LM}}: Friendly staff and clean environment.\\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}



  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{volume}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_volume_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Volume}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: Prices were very reasonable for the quality and quantity served.  \\
  \textbf{\textsc{Edit-then-Prototype}}: Prices were very reasonable for the quality and quantity of food there. \\
  \textbf{GPT-3}: The food was good, but the prices were a bit high for what \\
  \textbf{SSD-LM}: The manager seemed very pleased with the quantity and the good service. The manager was impressed by the price and quality. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The prices were quite reasonable for the quality and quantity of food that was presented. \\
  \textbf{\textsc{Cev-LM}}: And prices were surprisingly reasonable for the quality and quantity of food that was presented. \\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: I like this place--definitely going back. \\
  \textbf{\textsc{Edit-then-Prototype}}: I like going to this place for lunch. \\
  \textbf{GPT-3}: I really like this place. I'm definitely going back. \\
  \textbf{SSD-LM}: The service was quite good. The food was available and delicious for two hours. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Overall,everything was great and I'll be coming again next time. \\
  \textbf{\textsc{Cev-LM}}: Overall,had a great time and I'll definitely be back. \\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}



  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{circuitousness}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_circuitousness_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Circuitousness}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: I've only tried their Thai food,so far,and it is very good. \\
  \textbf{\textsc{Edit-then-Prototype}}: I've only tried their Thai food,so far,and it is very good. \\
  \textbf{GPT-3}: I've only tried their Thai food, so far, and it was really \\
  \textbf{SSD-LM}: They are very good in preparing food. However, if the food is really not good, then the chicken you can eat. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  \textbf{\textsc{Cev-LM}}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: I'd give the decor 4 stars and the food 3 stars. \\
  \textbf{\textsc{Edit-then-Prototype}}: I'd give the service 2 stars and the food 3 stars. \\
  \textbf{GPT-3}: I'd give the decor 3 stars and the food 4 stars. \\
  \textbf{SSD-LM}: The food was not well-priced and expensive, but very well-made, and I was very pleased with it. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: 3 stars for the food and 2 stars for the prices equals 2.5 stars for me. \\
  \textbf{\textsc{Cev-LM}}: I'd give 4 stars for the food and 3 stars for the service,3 stars for the decor. \\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}
  
% GPT3
% MuCoCo, Target Delta: 0.5, Delta: -2.86743, BERT: 72.425, BLEU: 0.0312
% SSD-LM, Target Delta: 0.5, Delta: -0.31998, BERT: 84.422, BLEU: 0.0581
